Time Varying Undirected Graphs

Undirected graphs are often used to describe high dimensional distributions. Under sparsity conditions, the graph can be estimated using $\ell_1$ penalization methods. However, current methods assume that the data are independent and identically distributed. If the distribution, and hence the graph, evolves over time then the data are not longer identically distributed. In this paper, we show how to estimate the sequence of graphs for non-identically distributed data, where the distribution evolves over time.

==> append-frob.tex <==
\section{Proof of Lemma~\ref{lemma:integral}}
\label{sec:append-frob}
The following proof is adapted from that of~\cite{RBLZ07}.
After factoring out $\twonorm{\mvec{\Delta}}^2 = \fnorm{\Delta}^2$,
LHS of the inequality becomes
\begin{eqnarray}
\nonumber
\lefteqn{\varphi_{\min}\left(\int^1_0(1-v)(\Theta_0 + v \Delta)^{-1}
\otimes (\Theta_0 + v \Delta )^{-1} dv\right) } \\ \nonumber
& \geq & 
\int^1_0 \varphi_{\min}\left((1-v)(\Theta_0 + v \Delta)^{-1}
\otimes (\Theta_0 + v \Delta)^{-1}\right) dv \\
\label{eq::kron-eigen}
& = & \int_0^1 (1-v)\varphi_{\min}^2(\Theta_0 + v \Delta)^{-1} dv \\ \nonumber
& \geq & 
\inf_{v \in [0, 1], \Delta \in \T_n} \varphi_{\min}^2 (\Theta_0 + v\Delta )^{-1} 
\int_0^1 (1-v) dv \\ \nonumber
& \geq & 
\inv{2} \inf_{\fnorm{\Delta'} \leq Mr_n,\Theta_0+ \Delta'\succ 0} 
\varphi_{\min}^2 (\Theta_0 + \Delta')^{-1} \\
& \geq & 
\frac{\underline{k}^2}{2 + \tau}, \text{ for }\tau = o(1).
\end{eqnarray}
where \eqref{eq::kron-eigen} is due to the fact that the set of $p^2$ eigenvalues 
of $B(v) \otimes B(v)$, where 
$B(v) = (\Theta_0 + v \Delta)^{-1}$, $\forall v \in [0, 1]$, 
$\forall \Delta \in \T_n$ 
is $\{\varphi_i(B(v)) \varphi_j(B(v)), \forall i, j =1, \ldots, p\}$,
which are all positive given that
$(\Theta_0 + v \Delta) \succ 0$, hence $(\Theta_0 + v \Delta)^{-1} \succ 0$,
$\forall v \in[0, 1], \forall \Delta \in \T_n$
as shown in Claim~\ref{claim:posi-def-interval}; and
the last step is due to the following:
$ \forall \Delta': \fnorm{\Delta'} \leq Mr_n$ such that 
$\Theta_0 + \Delta' \succ 0$,
\begin{eqnarray*}
\lefteqn{\varphi_{\min}(\Theta_0 + \Delta')^{-1} =
\inv{\twonorm{\Theta_0 + \Delta'}}}  \\
& \geq&
\inv{\left(\twonorm{\Theta_0}+ \twonorm{\Delta'}\right)} \geq 
\frac{\underline{k}}{1 + o(1)},
\end{eqnarray*}
where $\twonorm{\Delta'} \leq \fnorm{\Delta'}$ and 
$\inv{\ul{k}} \geq \twonorm{\Theta_0} = \Omega(2 Mr_n)$. 
$\Box$


